Unambiguous separators for tropical tree automata

In this paper we show that given a max-plus automaton (over trees, and with real weights) computing a function $f$ and a min-plus automaton (similar) computing a function $g$ such that $f\leqslant g$, there exists effectively an unambiguous tropical automaton computing $h$ such that $f\leqslant h\leqslant g$. This generalizes a result of Lombardy and Mairesse of 2006 stating that series which are both max-plus and min-plus rational are unambiguous. This generalization goes in two directions: trees are considered instead of words, and separation is established instead of characterization (separation implies characterization). The techniques in the two proofs are very different.

==> macros.tex <==
% !TEX root =  main-minmaxsep.tex

\let\leq\leqslant
\let\geq\geqslant


\newrobustcmd\sepc{\kl[\sepc]d}



\NewDocumentCommand\minautomaton{o}
  {\kl[\minautomaton]{\mathit{Min}}%
   \IfNoValueF{#1}{\kl[\autochange]{[}#1\kl[\autochange]{]}}}
\NewDocumentCommand\maxautomaton{o}
  {\kl[\maxautomaton]{\mathit{Max}}%
   \IfNoValueF{#1}{\kl[\autochange]{[}#1\kl[\autochange]{]}}}


\newrobustcmd\letter[1]{#1}
\newrobustcmd\lettera{\letter a}
\newrobustcmd\letterb{\letter b}

\newrobustcmd\word[1]{#1}
\newrobustcmd\wordu{\word u}
\newrobustcmd\wordv{\word v}
\newrobustcmd\wordw{\word w}

\newrobustcmd\state[1]{\kl[{\state #1}]{#1}}
\newrobustcmd\statep{\state p}
\newrobustcmd\stateq{\state q}
\newrobustcmd\stater{\state r}

\newrobustcmd\real[1]{#1}
\newrobustcmd\rx{\real x}
\newrobustcmd\ry{\real y}
\newrobustcmd\rz{\real z}



\newrobustcmd\automaton[1]{\mathcal{A}}   
\newrobustcmd\automatonA{\automaton A}   
\newrobustcmd\automatonB{\automaton B}   


\newrobustcmd\Alphabet{\mathtt{A}}
\newrobustcmd\initialVector{I}
\newrobustcmd\finalVector{F}
\newrobustcmd\transitions{\Delta}

\knowledgevariantmodifier{\intro*\intro}\intro

\newrobustcmd\integers{\mathbb{Z}}
\newrobustcmd\reals{\mathbb{R}}
\newrobustcmd\sem[1]{\kl[\sem]{[\![}#1\kl[\sem]{]\!]}}
\newrobustcmd\minsem[1]{\kl[\minsem]{[\![}#1\kl[\minsem]{]\!]}_{\min}}
\newrobustcmd\maxsem[1]{\kl[\maxsem]{[\![}#1\kl[\maxsem]{]\!]}_{\max}}
\newrobustcmd\States{{\kl[\States]Q}}
\newrobustcmd\minstates{\kl[\minstates]{\States}_{\kl[\minstates]{\minautomaton}}}
\newrobustcmd\maxstates{\kl[\maxstates]{\States}_{\kl[\maxstates]\maxautomaton}}
\newrobustcmd\mintransitions{\transitions_{\minautomaton}}
\newrobustcmd\maxtransitions{\transitions_{\maxautomaton}}
\newrobustcmd\mininitialstates{\kl[\mininitialstates]{I_{\minautomaton}}}
\newrobustcmd\minfinalstates{\kl[\minfinalstates]{F_{\minautomaton}}}
\newrobustcmd\maxinitialstates{\kl[\axinitialstates]{I_{\maxautomaton}}}
\newrobustcmd\maxfinalstates{\kl[\maxfinalstates]{F_{\maxautomaton}}}

\newrobustcmd\maxfinalweight{F_{\maxautomaton}}
\newrobustcmd\minfinalweight{F_{\minautomaton}}
\newrobustcmd\finalweight{F}
\newrobustcmd\initialweight{I}

\newrobustcmd\uautomaton{\mathcal{C}}

\newrobustcmd\trans[2]{\mathrel{\kl[\trans]{\rightarrow}^{#1}_{#2}}}
\newrobustcmd\maxtrans[1]{\trans{#1}{\maxautomaton}}
\newrobustcmd\utrans[1]{\trans{#1}{\uautomaton}}
\newrobustcmd\mintrans[1]{\trans{#1}{\minautomaton}}



\NewDocumentCommand\pprod{o}{%
   \IfNoValueTF{#1}
    {\mathrel{\kl[\pprod]{\odot}}}
    {\mathrel{\stackrel{#1}{\kl[\pprod[]]{\odot}}}}}
\newrobustcmd\refines{\mathrel{\kl[\refines]{\preccurlyeq}}}
\newrobustcmd\shiftrefines{\mathrel{\kl[\shiftrefines]{\preccurlyeq_{\mathtt{shift}}}}}
\newrobustcmd\closure[1]{\langle #1\rangle}
\newrobustcmd\closurek[2][k]{\langle #2\rangle^{\leq#1}}


\newrobustcmd\minmonoid{\kl[\minmonoid]{\mathcal{M}_{\min}}}
\newrobustcmd\maxmonoid{\kl[\maxmonoid]{\mathcal{M}_{\max}}}
\newrobustcmd\pmonoid{\kl[\pmonoid]{\mathcal{M}_{{\min}{\max}}}}
\newrobustcmd\powerset[1]{\mathcal{P}(#1)}




\newrobustcmd\PMidempotent[1]{\kl[\PMidempotent]{#1}}
\newrobustcmd\PMidempotentE{\PMidempotent E}

\newrobustcmd\threshold{\kl[\threshold]{t}}



% Semirings
\newrobustcmd\semiring[1][S]{\kl[\semiring]{\mathbf{#1}}}
\newrobustcmd\Identity{I}
\newrobustcmd\Reals{\mathbb{R}}
\newrobustcmd\Integers{\mathbb{Z}}
\newrobustcmd\pinfty{\kl[\pinfty]{+\infty}}
\newrobustcmd\minfty{\kl[\minfty]{-\infty}}
\newrobustcmd\Realspi{\Reals\uplus\{\pinfty\}}
\newrobustcmd\Realsmi{\Reals\uplus\{\minfty\}}
\newrobustcmd\Integerspi{\Integers\uplus\{\pinfty\}}
\newrobustcmd\Integersmi{\Integers\uplus\{\minfty\}}


\newrobustcmd\Cov{\kl[\Cov]{\mathit{Cov}}}


% pairs of matrices
\newrobustcmd\pmatrices[1]{#1}
\newrobustcmd\pmatricesK{\pmatrices K}


